Localisation principle for one-scale H-measures

Microlocal defect functionals (H-measures, H-distributions, semiclassical measures, etc.) are objects which determine, in some sense, the lack of strong compactness for weakly convergent ${\rm L}^p$ sequences. Recently, Luc Tartar introduced one-scale H-measures, a generalisation of H-measures with a characteristic length, which also comprehend the notion of semiclassical measures. We present a self-contained introduction to one-scale H-measures, carrying out some alternative proofs, and strengthening some results, comparing these objects to known microlocal defect functionals. Furthermore, we improve and generalise Tartar's localisation principle for these objects from which we are able to derive the known localisation principles for both H-measures and semiclassical measures. Moreover, we develop a variant of compactness by compensation suitable for equations with a characteristic length.

==> dodatak.tex <==
\def\Ljl#1{{{\rm L}^{2}_{{\rm loc}}(#1)}} 
\def\Ljlp#1{{{\rm L}^{p}_{{\rm loc}}(#1)}} 
\def\Ljli#1{{{\rm L}^{1}_{{\rm loc}}(#1)}} 
\def\Ljc#1{{{\rm L}^{2}_{{\rm c}}(#1)}} 
\def\buc#1{{\rm BUC}(#1)}
\def\Lpv#1{{{\rm L}^{p}_{{\rm #1}}}}
\def\Lpvd#1{{{\rm L}^{p}_{{\rm #1}}(\domena)}} 
\def\Lqv#1{{{\rm L}^{p'}_{{\rm #1}}}}
\def\Lqvd#1{{{\rm L}^{p'}_{{\rm #1}}(\domena)}} 
\def\Mx#1#2{{\rm M_{#1}}(#2)}

\def\L{{\rm L}}
\def\c{{\rm C}}
\def\S{{\rm S}}
\def\kobb{{\rm K_{0,\infty}}}
\def\kob#1{{{\rm K_{0,\infty}}}(#1)}
\def\Hlocn#1{{\rm H}_{{\rm loc}}^{-1}(#1)}
\def\Hlocp#1{{\rm H}_{{\rm loc}}^{1}(#1)}
\def\Hlocc#1{{\rm H}_{{\rm loc}}^{#1}}

\def\domena{\Omega}
\def\tdomena{\oi{0}{T}}

\def\skon{\rightharpoonup}

\def\ft#1{\lF{(#1)}}
\def\ftp#1{\lF{#1}}
\def\ftb#1{\lF{\bigl(#1\bigr)}}
\def\ftB#1{\lF{\Bigl(#1\Bigr)}}
\def\ift#1{\bar{\lF}(#1)}
\def\fp#1{\widehat{#1}}
\def\fpp#1{(#1)^\wedge}
\def\ifp#1{(#1)^\vee}
\def\erf{{\rm erf}}

\def\Dupp#1#2{\left\langle#1,#2\right\rangle}
\def\wt#1{\widetilde{#1}}

\def\szkon{\buildrel *\over\Dscon}
\def\Lbszkon{\buildrel \Lb\domena *\over\DDscon}
\def\LHh{\buildrel \Hlocn{\domena} \over\longrightarrow}
\def\postojij#1{(\exists!\,#1)}

%\def\binom#1#2{\Bigl(\matrix{
%#1 \cr
%#2 \cr}\Bigr)}
\def\binom#1#2{{#1\choose #2}}

\def\potpis#1#2{{%\vskip-3mm 
\narrower\smallskip\par
\noindent
{\bf Slika #1.} #2
\smallskip\par
}}

%%%%%%%%%%%%%% OZNAKE ZA MJERE %%%%%%
\def\hmv{\mmu_H}
\def\hm{\mu_H}
\def\pkmv{\mmu_{sc}}
\def\pkm{\mu_{sc}}
\def\jhm{\mu_\kobb}
\def\jhmv{\mmu_\kobb}


\newcount\bpr  \bpr=0
\outer\long\def\tv#1{\medbreak \global\advance\bpr by1
\noindent {\bf Tvrdnja \number\bpr.\enspace}{\sl #1 \par\smallbreak}}

\newcount\bnap \bnap=0
\outer\long\def\nap#1{\medbreak	\global\advance\bnap by1 
\noindent {\borgis {\bf Napomena \number\bnap.\enspace}{ #1 \hfill\kraj \par\medbreak}}}

\newcount\bsl \bsl=0
\outer\long\def\slutnja#1{\medbreak	\global\advance\bsl by1 
\noindent {\bf Slutnja \number\bsl.\enspace}{\sl #1 \hfill\kraj   \par\medbreak}}

\outer\long\def\tmcd#1#2{\medbreak	 \global\advance\btm by0
\noindent {\bf Teorem \number\btm.'\enspace}{\sl #1  \par\smallbreak} 
\noindent {\sf Dem.}\enspace #2 \par \hfill \hbox{\bf Q.E.D.}\par\medbreak} 

\newcount\bpr \bpr=0
\long\def\Primjerbr#1{{\medbreak	\global\advance\bpr by1
\noindent {\bf Primjer \number\bpr.\enspace }{ #1 \hfill\kraj   \par\medbreak} }} 

\def\im{{\sf im}\thinspace}

 

\endinput

